Multiple Instance Learning via Iterative Self-Paced Supervised Contrastive Learning

Learning representations for individual instances when only bag-level labels are available is a fundamental challenge in multiple instance learning (MIL). Recent works have shown promising results using contrastive self-supervised learning (CSSL), which learns to push apart representations corresponding to two different randomly-selected instances. Unfortunately, in real-world applications such as medical image classification, there is often class imbalance, so randomly-selected instances mostly belong to the same majority class, which precludes CSSL from learning inter-class differences. To address this issue, we propose a novel framework, Iterative Self-paced Supervised Contrastive Learning for MIL Representations (ItS2CLR), which improves the learned representation by exploiting instance-level pseudo labels derived from the bag-level labels. The framework employs a novel self-paced sampling strategy to ensure the accuracy of pseudo labels. We evaluate ItS2CLR on three medical datasets, showing that it improves the quality of instance-level pseudo labels and representations, and outperforms existing MIL methods in terms of both bag and instance level accuracy. Code is available at https://github.com/Kangningthu/ItS2CLR

==> macro.tex <==
\newcommand{\MAT}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\VEC}[1]{\left[\begin{array}{c} #1 \end{array}\right]}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\keys}[1]{\left\{ #1 \right\}}
\newcommand{\sqbr}[1]{\left[ #1 \right]}
\newcommand{\brac}[1]{\left( #1 \right) }
\newcommand{\ml}[1]{\mathcal{ #1 } }
\newcommand{\op}[1]{ \operatorname{#1} }
\newcommand{\normInf}[1]{\left\| #1 \right\| _{\infty}}
\newcommand{\normTwo}[1]{\left\| #1 \right\| _{2}}
\newcommand{\normOne}[1]{\left\| #1 \right\| _{1}}
\newcommand{\normTV}[1]{\left\| #1 \right\| _{\op{TV}}}
\newcommand{\normF}[1]{\left\| #1 \right\| _{F}}
\newcommand{\atomicnorm}[1]{\left\| #1 \right| \right|_{\mathcal{A}}}
\newcommand{\der}[2]{\frac{\text{d}#2}{\text{d}#1}}
\newcommand{\derTwo}[2]{\frac{\mathrm{d} ^2#2}{\mathrm{d}#1^2}}
% \newcommand{\set}[2]{ \keys{ #1 \; | \; #2 } }
\newcommand{\PROD}[2]{\left \langle #1, #2\right \rangle}
\newcommand{\diff}[1]{ \, \text{d} #1 }
\newcommand{\real}{\op{Re}}
\newcommand{\imag}{\op{Im}}
\newcommand{\wt}[1]{\widetilde{ #1 }}
\newcommand{\R}{\mathbb{R}}
\newcommand\at[2]{\left.#1\right|_{#2}}
\newcommand{\RR}{\mathcal{R}}



%Sheng
\usepackage[linesnumbered,ruled]{algorithm2e}
\newcommand\EE{\mathbb{E}}
\usepackage{graphicx}
\usepackage{amsmath, amssymb}
\usepackage{enumitem, array}
\usepackage[flushleft]{threeparttable}
%\usepackage{algorithm}% http://ctan.org/pkg/algorithms
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx

\newcommand{\Req}{\textbf{Require:}\hspace*{0.5em}}
\newcommand*\Let[2]{\State #1 $\gets$ #2}
\newcommand{\X}{\hspace*{3mm}}
\newcommand{\XX}{\X\X}
\newcommand{\XXX}{\X\X\X}
\newcommand{\XXXX}{\X\X\X\X}
\newcommand{\XXXXX}{\X\X\X\X\X}
\newcommand{\XXZ}{\XXX$\cdot${} }
\newcommand{\cm}[1]{$\triangleright$ #1}

\newcommand{\vy}{\mathbf{y}}
\newcommand{\vytrue}{\vy^*}
\newcommand{\va}{\mathbf{z}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\param}{\Theta}
\newcommand{\vone}{\mathbf{1}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vq}{\mathbf{t}}
\newcommand{\vv}{\mathbf v}
\newcommand{\vz}{\mathbf z}

\usepackage{xspace}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother

\usepackage{hyperref}
\hypersetup{hidelinks,
backref=true,
pagebackref=true,
hyperindex=true,
breaklinks=true,
colorlinks=true,%linkcolor=black,
urlcolor=blue,
bookmarks=true,
bookmarksopen=false,
pdftitle={Title},
pdfauthor={Author}}


\newcommand{\carlos}[1]{\textcolor{blue}{#1}}
\newcommand{\kangning}[1]{\textcolor{green}{#1}}
\newcommand{\sheng}[1]{\textcolor{violet}{#1}}

\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{multirow}
\usepackage{wrapfig}
